Structure Learning with Adaptive Random Neighborhood Informed MCMC

In this paper, we introduce a novel MCMC sampler, PARNI-DAG, for a fully-Bayesian approach to the problem of structure learning under observational data. Under the assumption of causal sufficiency, the algorithm allows for approximate sampling directly from the posterior distribution on Directed Acyclic Graphs (DAGs). PARNI-DAG performs efficient sampling of DAGs via locally informed, adaptive random neighborhood proposal that results in better mixing properties. In addition, to ensure better scalability with the number of nodes, we couple PARNI-DAG with a pre-tuning procedure of the sampler's parameters that exploits a skeleton graph derived through some constraint-based or scoring-based algorithms. Thanks to these novel features, PARNI-DAG quickly converges to high-probability regions and is less likely to get stuck in local modes in the presence of high correlation between nodes in high-dimensional settings. After introducing the technical novelties in PARNI-DAG, we empirically demonstrate its mixing efficiency and accuracy in learning DAG structures on a variety of experiments.

==> Neurips2023/old.tex <==
\section{Bayesian inference in structure learning}
\label{sec3:bayesstru}



% \subsection{Constraint-based methods and restricted spaces}


% The constraint-based methods rely on conditional independent testing. If it can be showed that two nodes are independent, given the data, conditioning on at least one set of the other nodes, the direct edge between these two nodes can then be excluded. The popular PC algorithm \citep{spirtes_2000_book} is to search for such undirected   the CPDAG of the Markov equivalence class.






% The PC algorithm is also adopted in some score and search methods (\textit{e.g.} the order/partition MCMC methods) to form hybrid schemes. Without the hybrid scheme, possible parent sets grow exponentially ($O(2^{p-1}$)), causing it to struggle in settings with $p \gg 20$ nodes \citep{sutter_2021, kuipers_2022}. Search over a restricted space leads to a biased scheme of which the MCMC sampler does not target the true posterior.

% We will use the restricted spaces in the following section in the pre-processing of the algorithmic tuning parameters. Although the , our scheme is still able to target the right distribution and unbiased sampler.  





















\subsection{Random neighborhood and informed proposals}
\label{sec:randneigh}




% As mentioned in earlier paragraphs, contributions on structure MCMC can be loosely differentiated between neighborhood methods that operate directly in the space of DAGs, and methods that restrict the search space by operating in transformed, smoother and lower capacity spaces of order or partitions using scoring functions. While our method falls into the first category, before describing the specifics, we briefly give an overview of both classes of methods and their advancements. 


% In this paper, all MCMC algorithms are Metropolis-Hastings based schemes \citep{metropolis1953equation,hastings1970monte}, which construct reversible Markov chains with invariant distribution coinciding with the target posterior distribution $\pi (\cdot)$. Let $\Gamma$ be the sample space and given a current DAG $\gamma^{(t)} \in \Gamma$ at time $t$, a new DAG $\gamma^\prime$ is proposed according to some proposal kernel $Q(\gamma^{(t)}, \cdot)$ with mass function $q$, and accepted as the next state $\gamma^{(t+1)}$ with acceptance probability
% \begin{align}
%     \alpha(\gamma^{(t)}, \gamma^\prime) = \min\left\{1, \frac{\pi(\gamma^\prime)q(\gamma^\prime,\gamma^{(t)})}{\pi(\gamma^{(t)})q(\gamma^{(t)}, \gamma^\prime)}\right\}. 
% \end{align}




We begin by introducing the class of random neighborhood proposals for Bayesian structure learning problems. A random neighborhood proposal normally involves two steps: randomly sample a neighborhood $\mathcal{N}$, then propose a new DAG within this neighborhood $\mathcal{N}$. To describe the distribution of the neighborhoods $\mathcal{N}$ conditional on current $\gamma$, we assume that the randomness in sampling $\mathcal{N}$ can be interpreted as stemming from an auxiliary \emph{neighborhood indicator} variable $k \in \mathcal{K}$, with conditional distribution $p(\cdot|\gamma)$, such that the neighborhood is constructed as a function of $\mathcal{N}(\gamma, k)$. The new proposal $\gamma^\prime \in \mathcal{N}(\gamma, k)$ is then drawn from the distribution $q_k(\gamma, \cdot)$. The random neighborhood proposal takes the form of \textit{Metropolis-Hastings} (MH) scheme \citep{metropolis1953equation,hastings1970monte} which constructs a $\pi$-reversible chain. In the reverse proposal, we consider a deterministic self-inverse mapping $k^\prime = \rho(k)$ (see Section 3.1 of \cite{liang2022adaptive} for detailed discussions). The full update of a single iteration of a generic random neighborhood proposal include:
\begin{enumerate}[label= \roman*), leftmargin=5ex]
    \item \emph{Neighborhood construction}: sample $k$ according to $p(\cdot|\gamma)$ and construct $\mathcal{N}(\gamma, k)$.
    \item \emph{Within-neighborhood proposal}: propose a new model $\gamma^\prime \sim q_k(\gamma, \cdot)$ in $\mathcal{N}(\gamma, k)$.
    \item \emph{Accept/reject step}: Update $k^\prime = \rho(k)$ and compute the reverse probability $q_{k^\prime}(\gamma^\prime, \gamma)$. Accept $\gamma^\prime$ with probability 
    \begin{align} \small
        \alpha_k(\gamma, \gamma^\prime) = \min\left\{1, \frac{\pi(\gamma^\prime)p(k^\prime|\gamma^\prime)q_{k^\prime}(\gamma^\prime, \gamma)}{\pi(\gamma)p(k|\gamma)q_k(\gamma, \gamma^\prime)}\right\}.
    \end{align}
\end{enumerate}


% \begin{example}[ADR sampler]
    % Add-Delete-Reverse scheme \citep{madigan1995bayesian, giudici2003improving} is a random neighborhood sampler where the space of neighborhood indicator $k$ contains three moves $\mathcal{K} = \{\text{``Add''}, \text{``Delete''}, \text{``Reverse''}\}$. The neighborhood indicator $k$ is uniformly distributed over the space $\mathcal{K}$, and the within-neighborhood proposal uniformly proposes a new DAG in $N(\gamma, k)$. The mapping $\rho(k)$ sends $k$ to its reverse move (\textit{e.g.} it opposes an addition move to a deletion move, and vice versa).
% \end{example}

A typical case of a random neighborhood sampler for Bayesian structural learning is represented by the Add-Delete-Reverse (ADR) proposal \citep{madigan1995bayesian, giudici2003improving}. In ADR, the neighborhood indicator $k$ is defined by three possible moves in the space $\mathcal{K} = \{\text{`Add'}, \text{`Delete'}, \text{`Reverse'}\}$. Once $k$ is uniformly drawn from $\mathcal{K}$, a new model DAG $\gamma^\prime$ is proposed from the neighborhood $\mathcal{N}(\gamma, k)$ with uniform probability. 



The main issues of ADR are associated with its slow mixing, as it is hard for the random walk proposal to explore important neighborhoods of edges in high-dimensions as it is likely to get stuck in neighborhoods with highly correlated nodes. The recent work of \cite{zanella2020informed} has shed light on how to construct efficient MCMC proposals in discrete space by introducing the \textit{locally informed proposal}. This can be used in the random neighborhood framework outlined above to replace the within-neighborhood random walk proposal $q_k (\gamma, \cdot)$ with a new proposal $q_{g,k}(\gamma, \cdot)$, which re-weights $q_k(\gamma, \cdot)$ according to the target distributions to facilitate moves to more promising candidate DAGs and speed up convergence. This is done by means of a monotonous and continuous balancing function $g:[0, \infty) \to [0, \infty)$, which satisfies $g(x) = xg(1/x)$. The new informed within-neighborhood proposal has the following form 
\begin{align} 
    q_{g,k} (\gamma, \gamma^\prime) = 
    \frac{1}{Z_{g,k}(\gamma)}g\left( \frac{\pi(\gamma^\prime)p(k^\prime|\gamma^\prime)}{\pi(\gamma)p(k|\gamma)} \right) \mathbb{I}\left\{\gamma^\prime \in \mathcal{N}(\gamma, k)\right\} ~ , \label{mat:within-informed}
\end{align}
where $Z_{g,k}(\gamma)$ is the normalising constant and $k^\prime = \rho(k)$. The associated acceptance probability is given by 
\begin{align*}
    \alpha_{g,k}(\gamma, \gamma^\prime) = \min \left\{1 , \frac{\pi(\gamma^\prime)p(k^\prime|\gamma^\prime)q_{g,k^\prime}(\gamma^\prime, \gamma)}{\pi(\gamma)p(k|\gamma)q_{g,k}(\gamma, \gamma^\prime)}\right\}.
\end{align*}
In this work, we only consider the Hastings' choice (\textit{i.e.} $g(x) = \min\{1,x\}$) which is the stablest choice for most of the problems (see the discussion in Supplement B.1.3 of \cite{zanella2020informed}). The informed proposal here not only helps speed up convergence, but it also avoids proposing invalid DAGs. The acyclicity checks for candidate models $\gamma^\prime \in \mathcal{N}(\gamma, k)$ can be run before computing their posterior model probability, and thus assign zero mass to their prior (resulting in zero mass posterior) if $\gamma^\prime$ is not a valid DAG.







\subsection{Point-wise implementation of Adaptive Random neighborhood informed proposal}


Recently, \cite{liang2022adaptive} introduced the Point-wise Adaptive Random Neighborhood Informed proposal (PARNI) in the context of Bayesian variable selection problems. The PARNI proposal couples the Adaptively scaled Individual Adaption scheme \citep{griffin2021search} with the random neighborhood informed proposal described above. In this work, we non-trivially tailor it specifically to the problem of DAGs sampling (resulting in the PARNI-DAG proposal). 

We begin by defining $k$ and $\mathcal{N}(\gamma, k)$ used in PARNI. The dimension of $k$ complies with the dimension of $\gamma$ (\textit{i.e.} $\mathcal{K} = \Gamma = \{0,1\}^{n \times n}$), and each position in $k$ indicates whether the corresponding position in $\gamma$ is included in the neighborhood. If $k_{ij} = 1$, $\gamma_{ij}$ is included in the neighborhood, otherwise $\gamma_{ij}$ is not included. The conditional distribution of $k$ takes a product form $p_{\eta}(k|\gamma) = \prod_{i,j} p_{\eta}(k_{ij}|\gamma_{ij})$, characterized by the set of tuning parameters $\eta = \{\eta_{ij}\}_{i,j=1}^n$, where $\eta_{ij} \in (\epsilon, 1-\epsilon)$ for a small $\epsilon \in (0, 1/2)$, and is given by
\begin{align} \small
    p_{\eta}(k_{ij} = 1|\gamma_{ij} = 0) = \min\left\{1,\frac{1 - \eta_{ij}}{\eta_{ij}}\right\}~, \quad  p_{\eta}(k_{ij} = 1|\gamma_{ij} = 1) = \min\left\{1,\frac{\eta_{ij}}{1-\eta_{ij}}\right\}~.  \label{mat:PARNI_RN}
\end{align}
\cite{griffin2021search} and \cite{liang2022adaptive} both suggest using the posterior inclusion probabilities in Bayesian variable selection, the equivalent of \textit{posterior edge probabilities} (PEP) in our case, i.e.~$\pi(\gamma_{ij} = 1)$, to define $\eta_{ij}$. The distribution (\ref{mat:PARNI_RN}), with this choice of parameters, encourages to flip these variables based on their marginal importance. Suppose $\pi(\gamma_{ij} = 1) = 0.9$ and the chain is currently at $\gamma_{ij} = 0$, the edge should be assigned higher probability to be included in the DAG ($\gamma_{ij}$ switched from 0 to 1). Thus we propose $k_{ij} = 1$ with probability $\min\{1, 0.9/0.1\} = 1$, so that $\gamma_{ij}$ will be switched in the next stage. The other advantage of using the conditional distribution in (\ref{mat:PARNI_RN}) is that it is a perfect sampling scheme as it draws samples directly from the posterior, provided that all variables are independent, and achieves optimal asymptotic variance \citep{griffin2021search}.




To construct the new neighborhood defined by $\mathcal{N}(\gamma, k)$ according to the above, we should be able to propose a new $\gamma^*$ where the $(i,j)$ entries must be different than $\gamma$, such that their corresponding neighborhood indicator is $k_{ij} = 1$, otherwise we stick to $\gamma^*_{ij} = \gamma_{ij}$, namely:
\begin{align}
    \mathcal{N}(\gamma, k) = \left\{\gamma^* \in \Gamma \mid \, \gamma^*_{ij} = \gamma_{ij} ~ \forall (i,j) ~ \text{s.t.} ~ k_{ij} = 0 \right\}.
\end{align}
Technically, a simple random neighborhood informed proposal can then be constructed with the above choice of $k$ and neighborhood $\mathcal{N}(\gamma, k)$, and with the informed within-neighborhood proposal as in (\ref{mat:within-informed}). However, in practice, given the neighborhood size $d_k = \sum_{ij} k_{ij}$, there are $2^{d_k}$ possible DAGs within $\mathcal{N}(\gamma, k)$, growing exponentially with $d_k$. The full enumeration over the whole neighborhood is computationally expensive when $d_k$ is big. For example, consider the \texttt{gsim100} simulated data in \cite{suter2021bayesian}, with 161 true edges. The average size of $k$ is above 320 and thus it includes $\gg 2^{320}$ DAGs. 

A point-wise implementation \citep{liang2022adaptive} is helpful in this case. The idea is that, instead of working with the full $\mathcal{N}(\gamma, k)$ neighborhood, we construct a sequence of small neighborhoods $\{\mathcal{N}(\gamma(r), K_r)\}_{r=1}^R \subset \mathcal{N}(\gamma, k)$, and a new DAG $\gamma^\prime$ is sequentially proposed from these neighborhoods $\{\mathcal{N}(\gamma(r), K_r)\}_{r=1}^R$ according to the sub-proposals $q_{K_r}(\gamma(r-1), \cdot)$ at each time $r$ where $\gamma = \gamma(0) \to \gamma(1) \to \dots \to \gamma(R) = \gamma^\prime$ are intermediate models. The new model indicator $K_r$ represents the collection of positions where $k_{ij} = 1$. In the original PARNI proposal, each $K_r$ only contains one single position $(i,j)$, so that each sequential small neighborhood only contains 2 models, which allows one component of $\gamma$ to switch. The computational time is therefore reduced dramatically from $\mathcal{O}(2^{d_k})$ to $\mathcal{O}(2 d_k)$. More details on point-wise implementation are given in the supplementary material (Appendix D).


In the next section, we propose a new $K_r$, introduce a reversal neighborhood move and few more new components in PARNI that are specifically tailored for the problem of DAG sampling.






\section{The novel PARNI-DAG proposal and motivations}


\subsection{Pre-computing $\eta$ under restricted space and its adapting scheme}

Let $\gamma_{-ij}$ denote any other edge excluding the $\gamma_{ij}$ edge. For the tuning parameter $\eta$ defined in the previous section, \cite{griffin2021search} and \cite{liang2022adaptive} consider a Rao-Blackwellised estimation of the posterior inclusion probabilities $\pi(\gamma_{ij} = 1|\gamma_{-ij})$, updated on the fly given the output of the chain. The Rao-Blackwellisation is however infeasible in the context of DAG sampling because it entails computing $n^2$ model probabilities. Also, updating $\eta$ based on the marginal sum over the output $\{\gamma^{(l)}\}_{l=1}^t$ as
\begin{align}
    \hat{\pi}^{(t)}_{ij} = \frac{1}{t} \sum_{l = 1}^t \mathbb{I} \left\{ \gamma_{ij}^{(l)} = 1 \right\}
\end{align}
would be too slow to converge. This updating scheme also leads to other issues such as poor exploration and mis-specification of the important edges. It is worth mentioning that $\eta$'s do not have to be the exact PEPs, as we can still draw valid samples from the target posterior distribution $\pi$ as long as the MH acceptance probability preserves $\pi$-reversibility. However, choosing $\eta$'s that are close to the true PEPs will cause each component to change and to target the right proportion of their marginal probabilities (higher probability of including important edges). 


Our solution is to approximate the PEPs $\Tilde{\pi}_{ij}$ before running the PARNI-DAG algorithm and use the approximation to warm-start the chain. While running the algorithm at time $t$, we update the tuning parameters $\hat{\eta}^{(t)}_{ij}$ adaptively based on
\begin{align}
    \hat{\eta}^{(t)}_{ij} = \phi_t \Tilde{\pi}_{ij} + (1-\phi_t) \hat{\pi}^{(t)}_{ij}
\end{align}
where $\{\phi_l\}_{l=1}^t$ is a decreasing sequence which controls the trade-off between warm-start PEPs $\Tilde{\pi}_{ij}$ and marginal sum of the output $\hat{\pi}^t_{ij}$. The choice of $\{\phi_l\}_{l=1}^t$ is not unique and we give a full specification of our choice in the supplementary material (Appendix B). In the following, we will briefly describe the methods used to calculate the warm-start approximation $\Tilde{\pi}_{ij}$.









We find the restricted space technique from the hybrid schemes \citep{kuipers_2022} particularly useful in a priori deleting the most unlikely DAG models, and thus efficiently approximating the PEPs. Let $\mathcal{H}$ be the skeleton (not necessarily acyclic) obtained from either PC algorithm or other search space scheme (\textit{e.g.} the end space of the iterativeMCMC algorithm). Adopting the same notations as in \cite{kuipers_2022}, the resulting adjacency matrix $H$ must satisfy $H_{ij} = 1$ if $(i,j)$ is an edge of $\mathcal{H}$. For node $X_j$, the adjacency matrix $H$ defines the \textit{permissible parent set} $h^j = \left\{X_{i}: ~ H_{ij} = 1\right\}$. All possible parent combinations of node $X_j$ is concluded in the \textit{collection of permissible parent set} which is defined by
\begin{align}
    \mathbf{h}^j = \{ m |~ m \subseteq h^j \}.
\end{align}
The collection of permissible parent set $\mathbf{h}^j$ can be then extended to a bigger collection $\mathbf{h}^j_+$ as described in Section 4.3 of \cite{kuipers_2022}. Basically, the extended collection of permissible parent set $\mathbf{h}^j_+$ also includes one other node from outside the permissible parent set $h^j$ as an additional parent, otherwise the candidate parents of $X_j$ are restricted to those nodes are connected directly to $X_j$ in adjacency matrix $H$. We then approximate $\Tilde{\pi}_{ij}$ in the following procedure:
\begin{enumerate}[leftmargin=4ex]
    \item Dropping the acyclicity constraint from the prior (\ref{mat:prior}) and forming the unconstrained posterior distribution $\pi^u(\gamma)$, approximating the marginal probability $\pi^u(\gamma_{ij})$ under $\mathbf{h}^j_+$.
    \item Approximating the joint probability of pair edges by the product
    \begin{align}
        \Tilde{\pi}(\gamma_{ij}, \gamma_{ji}) \approx \pi^u(\gamma_{ij}) \times \pi^u(\gamma_{ji})
    \end{align}
    \item Imposing back the simplest acyclicity constraint which avoids creating two edges with opposite directions, \textit{i.e.} let $\Tilde{\pi}(\gamma_{ij} = 1, \gamma_{ji} = 1) = 0$. Approximating 
    \begin{align}
        \Tilde{\pi}_{ij} = \frac{\Tilde{\pi}(\gamma_{ij} = 1, \gamma_{ji} = 0)}{\Tilde{\pi}(\gamma_{ij} = 1, \gamma_{ji} = 0) + \Tilde{\pi}(\gamma_{ij} = 0, \gamma_{ji} = 1) + \Tilde{\pi}(\gamma_{ij} = 0, \gamma_{ji} = 0)}.
    \end{align}
\end{enumerate}
The detailed of the whole calculations of $\Tilde{\pi}_{ij}$ is given in the supplementary material (Appendix C).










\subsection{Introducing the ``reversal'' neighborhood}


It is natural that a pair of edges $i \longleftrightarrow j$ is highly correlated and they could be both included in a DAG. This correlation structure also explains the mixing improvements of ADR proposal over the $\text{MC}^3$ proposal. In the classic PARNI proposal, each $K_r$ corresponds to exactly one position $(i,j)$ such that $k_{ij} = 1$, and it does not support the reversal move in one single sub-proposal $q_{K_r}$. Suppose that currently $\gamma_{ij} = 1$ and $\gamma_{ji} = 0$, to propose a reversal move according to the classic PARNI proposal, we should first propose to remove $\gamma_{ij}$ from the DAG, then include $\gamma_{ji}$ in the following sub-proposals. These flips might be running into issues if the posterior model probability for excluding both edges, $\gamma_{ij} = \gamma_{ji} = 0$, is low, so that these moves are rarely proposed and the chain gets stuck at $\gamma_{ij} = 1$. 


One solution to tackle this issue is to construct a bigger neighborhood which contains the edge reversal move of a DAG in PARNI. This development allows for the edge reversal move within single sub-proposal without going through the low posterior probabilistic models and avoids the chain getting stuck. At each iteration of the Markov chain, suppose $k$ is the sampled. For all those pairs which satisfy $k_{ij} = 1$ and $k_{ji} = 1$ in $k$, we construct the reversal neighborhoods for edges $\gamma_{ij}$ and $\gamma_{ji}$. For the rest of positions that $k_{ij} = 1$ but $k_{ji} = 0$, we construct the original neighborhood which only contains the current model and model with $\gamma_{ij}$ flipped. The idea of this reversal neighborhood is merged to the main PARNI-DAG proposal given in the supplementary material (Appendix D). 










\subsection{New adapting scheme involving computational efficiency}


Although the point-wise implementation has reduced the per-iteration costs from exponential to linear to the neighborhood size (equivalent to number of sub-neighborhoods in PARNI), the PARNI proposal is still computationally expensive if the sampled DAGs are not very sparse. Recall the \texttt{gsim100} dataset, we often require computing 320 posterior model probabilities on average in one iteration of MCMC and the computation thus becomes 320 times more expensive than the ADR proposal. We make use the neighborhood thinning parameter $\omega$ in the original PARNI in a slight different way, to control the number of neighborhoods evaluated and reduce computational cost, which eventually improves computational efficiency.




In the original PARNI proposal, the thinning parameter $\omega$ represents the random walk jumping probability without taking the posterior model probabilities into account. It does not affect the number of neighborhoods evaluated. But for the new PARNI-DAG proposal, with probability $1-\omega$, we will skip some neighborhoods. Within each iteration, for each time $r$, given the current proposal $\gamma(r-1)$ and neighborhood indicator $K_r$, the PARNI-DAG proposal does:
\begin{enumerate}[leftmargin=3ex]
    \item With probability $\omega$, proposal $\gamma(r) \sim q_{K_r}(\gamma(r-1), \cdot)$ where 
    \begin{align} 
        q_{K_r}(\gamma(r-1), \gamma(r)) \propto g\left(\frac{\pi(\gamma(r))p(K_r|\gamma(r))}{\pi(\gamma(r-1)p(K_r|\gamma(r-1)))}\right) \mathbb{I} \{\gamma(r) \in \mathcal{N}(\gamma(r-1), K_r)\}.
    \end{align}
    \item With probability $1-\omega$, the posterior probabilities for other DAGs in $\mathcal{N}(\gamma(r-1), K_r)$ are not evaluated and directly propose $\gamma(r) = \gamma(r-1)$.
\end{enumerate}
Controlling $\omega$ can vary the number of posterior model probability evaluations. Larger the value of $\omega$, more model probabilities are required to compute. If $\omega = 1$, all neighborhoods are required to propose a new DAG. 

The $\omega$ is updating adaptive. Here, we consider the Robins-Monro adaptation scheme on updating the tuning parameter $\omega$ on the fly. At time $t$, the new parameter is updated by
\begin{align}
    \text{logit}_\epsilon \omega^{(t+1)} = \text{logit}_\epsilon \omega^{(t)} - \psi_t (\mathcal{N}_t - \Tilde{\mathcal{N}})
\end{align}
where $\mathcal{N}_t$ is number of sub-neighborhoods evaluated at time $t$ and $\Tilde{\mathcal{N}}$ is a pre-specified expected number of evaluations. We set $\psi_t = t^{-0.7}$ which implies the adaptation of $\omega$ diminishes at the rate of $\mathcal{O}(t^{-0.7})$. From empirical results, we find that targeting 10 neighborhoods on average can achieve optimal balance between the mixing performance and computational cost, it also supports for certain degrees of exploration that proposes reasonable amount of changes. Therefore, we set $\Tilde{\mathcal{N}} = 10$ for all numerical studies in Section \ref{sec5:simulations} and supplementary material (Appendix F).









\subsection{Why PARNI-DAG?}

To conclude this section, we briefly summarize the strengths of PARNI-DAG with respect to other existing MCMC methods for structure learning. Firstly, as already discussed in previous sections, PARNI-DAG has clear advantages compared to ADR in terms of speed of convergences and mixing, while targeting the same posterior distribution of DAGs. As for score-based MCMC methods, order MCMC \citep{friedman_2003} has better scalability than standard structure MCMC such as MC$^3$, but it works in the space of orders and not DAGs, and it introduces sampling bias by placing a non-uniform prior on some DAGs which are compatible with multiple orders \citep{ellis2008learning}. \cite{kuipers_2017} proposes a variant called partition MCMC, which operates in the space of ordered partitions. Partition MCMC is unbiased in terms of sampling, but it is extremely slow as it has very high computational complexity, and can only be used on very few nodes \citep{kuipers_2022}. Compared to order MCMC, PARNI-DAG does not incur in any sampling bias as it targets the posterior on DAGs directly, while at the same time converging faster than ADR.





The hybrid MCMC scheme of \cite{kuipers_2022} proposes to restrict the search space by pruning it via a skeleton graph (e.g.~PC skeleton) $\mathcal{H}$, whose max parent set size is $m$ per node, so that complexity reduces to $O(n 2^m)$. Although this increases MCMC speed dramatically in large graphs, it is likely to introduce bias as some true edges might be deleted in $\mathcal{H}$. To tackle this issue they also propose an iterative procedure to re-populated $\mathcal{H}$ with additional potential parent nodes, but this increases computational time. PARNI-DAG instead uses a previously derived skeleton $\mathcal{H}$ not to restrict the space, and possibly cancel out relevant edges, but only to warm-start the chain by pre-tuning the $\eta$ parameters as explained earlier in this section.






%\subsection{Order and partition MCMC}

%The other class of structure MCMC samplers reviewed here relies on DAG scoring measures where $p(\mathcal{G} | \mathcal{D}) = \prod^n_{j=1} S( X_j, \text{Pa}(X_j) | \mathcal{D} ) $, and on restricting the search space of DAGs to some lower capacity set. \cite{friedman_2003} first proposed order MCMC, which operates in the space of orders $(\bm{X}, \prec)$ instead of the DAG one. This search space is smoother, so that order MCMC generally achieves faster convergence with respect to classic neighborhood MCMC. The method considers permutations $(j_1, ..., j_d)$ of nodes that imply a linear order $j_1 \prec ... \prec j_d$. Each linear order is then given a score $R( \prec | \mathcal{D})$ equal to the sum of scores of all the compatible DAGs with the order $\prec \, \in (\bm{X}, \prec)$. To restrict the space capacity even more, sum and product operations can be swapped so that the order's score is:
%\begin{equation*}  \small
%\begin{split}
%    R( \prec | \mathcal{D}) = \sum_{\mathcal{G} \in \prec} p(\mathcal{G} | \mathcal{D}) & \propto \sum_{\mathcal{G} \in \prec} \prod^d_{j=1} S( X_j, \text{Pa}(X_j) | \mathcal{D} )  \\
%    & \propto \prod^d_{j=1} \sum_{\text{Pa} (X_j) \in \prec } S( X_j, \text{Pa}(X_j) | \mathcal{D} ) \, ,
%\end{split}
%\end{equation*}
% where $S(\cdot)$ is a DAG scoring function, such as the Bayesian Gaussian equivalent (BGe) score for continuous variables \citep{geiger2002parameter}. Constructing a MCMC in the space of orders means moving from order $\prec$ to order $\prec'$ with MH acceptance probability $\alpha_{\prec} ( \prec, \prec' ) = \min \left\{ 1, \frac{R(\prec^\prime | \mathcal{D})}{R(\prec | \mathcal{D})} \right\}$, according to following moves: a) ``Local Swap" swaps adjacent nodes in $\prec$; b) ``Global Swap" swaps random nodes in $\prec$; c) ``Relocate" picks a node and replaces it in all possible positions in $\prec$, while keeping the rest of the order unchanged. Order MCMC is efficient, but has two main drawbacks compared to neighborhood MCMC: i) it outputs a sample of orders, not a DAG directly; sample of DAGs can be obtained by sampling, for each node independently, a parent set compatible with the relative order $\prec$, thanks to score decomposability (then get the DAG with maximum score in the sample as MAP estimate); ii) Order MCMC places a non-uniform prior on some DAGs by over-representing them in more than one order $\prec$, which causes the sample to be biased \citep{ellis2008learning}. 

% In the attempt to correct sampling bias, \cite{kuipers_2017} proposes a variant called partition MCMC, which operates in the space of ordered partitions instead. A labelled partition $\Lambda$ is a pair of order $\prec$ and partitioning vector $\bm{\delta} = (\delta_1, ..., \delta_p)$ where $p < d$, and $\sum^p_{j=1} \delta_j = d$. Vector $\bm{\delta}$ divides the order into $p$ parts $v_1, ..., v_p$ such that $v_1$ contains the first $\delta_1$ nodes of the order $\prec$ and so on. A DAG is compatible with partition $\Lambda = (\prec, \bm{\delta})$ if for every node $X_j \in v_j$: i) $X_j$ has at least one parent in part $v_{j+1}$; ii) all $\text{Pa}(X_j)$ belong to parts with indices higher than $j$; iii) $\text{Pa}(X_j) = \emptyset$ only if $j=p$. The possible moves of partition MCMC are: a) swap 2 nodes from different parts; b) swap 2 nodes from adjacent parts; c) split or join two parts; d) move a node in another existing part or create a new part with that node. Partition MCMC is unbiased in terms of DAG sampling; however it is extremely slow as it has very high computational complexity, and therefore can only be used to sample DAGs with very few nodes \citep{kuipers_2022}. 








==> Neurips2023/table.tex <==
\begin{table*}[t]
    \centering
    \ra{1.2}
    \scalebox{0.9}{
    \begin{tabular}{c|c|c|c|c}
    \toprule
            & \textbf{ecoli70} & \textbf{magic-niab} & \textbf{magic-irri} & \textbf{arth150}  \\
         \midrule
         \textbf{PC} & 62.65 $\pm$ 1.64 & 66.95 $\pm$ 0.82 & 103.75 $\pm$ 0.91 & 126.70 $\pm$ 2.10 \\
         \textbf{GES} & 47.95 $\pm$ 1.72 & 65.50 $\pm$ 0.42 & 97.60 $\pm$ 0.99 & 129.70 $\pm$ 3.47 \\
         \textbf{LiNGAM} & 107.4 $\pm$ 3.96 & 71.60 $\pm$ 1.34 & 111.25 $\pm$ 2.34 & -  \\
         \textbf{Order MCMC} & 42.85 $\pm$ 1.30 & \textbf{62.05 $\pm$ 1.52} & \textbf{92.90 $\pm$ 1.46} & 110.00 $\pm$ 1.96 \\
         \textbf{Iterative MCMC} & \textbf{39.55 $\pm$ 2.15} & 65.00 $\pm$ 2.43 & 96.15 $\pm$ 2.11 & 119.45 $\pm$ 3.43 \\
         \textbf{Partition MCMC} & 48.85 $\pm$ 2.76 & 66.20 $\pm$ 1.62 & 103.35 $\pm$ 1.81 & 140.75 $\pm$ 4.04 \\
         \textbf{ADR} & \textbf{39.40 $\pm$ 1.27} & 64.25 $\pm$ 0.64 & 95.20 $\pm$ 1.16 & 143.15 $\pm$ 1.62 \\
         \textbf{PARNI-DAG} & \textbf{37.55 $\pm$ 1.59} & \textbf{64.14 $\pm$ 0.55} & \textbf{91.85 $\pm$ 0.97} & \textbf{97.60 $\pm$ 2.16} \\
         \bottomrule
    \end{tabular}
    }
    \caption{SHD averaged over $20$ replications with associated 95\% confidence intervals of the various models compared on the four datasets ($n = 100$). All algorithms were ran for approximately the same CPU-time and the significantly best performing models are given in \textbf{bold}. (\textit{Lower is better.})}
    \label{tab:bnlearn}
\end{table*}

